Electroweak Corrections at High Energies

We present a survey of the most abundant processes at the LHC for sensitivity to electroweak corrections at \sqrt{s} = 8, 14, 33, and 100 TeV proton-proton collision energies. The processes studied are pp -> dijet, inclusive W and Z, W/Z+jets, and WW. In each case we compare the experimental uncertainty in the highest kinematic regions of interest with the relative magnitude of electroweak corrections and fixed-order \alpha_S calculations.

==> TotCS-ptl-cuts_ZNul_LHC100_mstw.dat.tex <==
 % Total cs for different cuts at the LHC       
 %************************************************
 % PDFs : mstw
 % p_{\rT,miss}^{\mathrm{min}}/(\GeV)            &                100.0 &                200.0 &                400.0 &                800.0 &               2000.0 &               4000.0 \\ 
 %-------------------------------------------------
                            $$ \begin{array}{c|rrrrrr}
                                                                  \multicolumn{7}{c}{\Pp\Pp
                                                                    \to l^+l^-\; \mathrm{jet} + X \;\mbox{at} \;\sqrt{s} =100 \TeV} \\
              \hline p_{\rT,l^+} / \GeV & 100-\infty \;\;\; & 200-\infty \;\;\; & 400-\infty \;\; & 800-\infty \;\; & 2000-\infty \;\; & 4000-\infty \; \\ 

 \hline \hline 
                 \si_{\born}^{\mu = \MZ}/\pba \; & \;              44.075(8)                  \; & \;               6.865(1)                  \; & \;              0.9684(1)                  \; & \;             0.11379(2)                  \; & \;           0.0045639(8)                  \; & \;          0.00024532(5)                  \\ 
              \si_{\born}^{\mathrm{var}}/\pba \; & \;              45.107(9)                  \; & \;               6.643(1)                  \; & \;              0.8362(1)                  \; & \;             0.08329(1)                  \; & \;           0.0025868(5)                  \; & \;          0.00011752(3)                  \\ 
 %--------------------------------------------------
 %--------------------------------------------------
  \hline \hline 
                   \de_{\EW}^{\mu = \MZ} / \% \; & \;               -9.68(2)                  \; & \;              -14.56(3)                  \; & \;               -22.5(3)                  \; & \;               -31.1(1)                  \; & \;               -44.5(3)                  \; & \;               -51.8(8)                  \\ 
    \de_{\EW}^{\mathrm{rec}\,,\mu = \MZ} / \% \; & \;               -6.53(5)                  \; & \;              -11.17(4)                  \; & \;              -18.17(6)                  \; & \;               -26.8(1)                  \; & \;               -39.8(2)                  \; & \;                -49.(1)                  \\ 
 %--------------------------------------------------
 \hline 
                  \de_{\EW}^{\mathrm{var}}/\% \; & \;               -9.54(2)                  \; & \;              -14.22(3)                  \; & \;              -21.20(6)                  \; & \;               -29.6(2)                  \; & \;               -41.8(8)                  \; & \;               -41.8(6)                  \\ 
   \de_{\EW}^{\mathrm{rec}\,,\mathrm{var}}/\% \; & \;               -6.32(6)                  \; & \;              -10.81(4)                  \; & \;              -17.38(6)                  \; & \;               -25.1(1)                  \; & \;                -39.(1)                  \; & \;               -35.4(8)                  \\ 
 %--------------------------------------------------
 %--------------------------------------------------
  \hline \hline 
                    \de_{\QCD}^{\mu = \MZ}/\% \; & \;                73.6(3)                  \; & \;                77.4(2)                  \; & \;                68.2(2)                  \; & \;                41.1(2)                  \; & \;               -20.5(6)                  \; & \;               -75.2(8)                  \\ 
                 \de_{\QCD}^{\mathrm{var}}/\% \; & \;                60.1(4)                  \; & \;                62.5(2)                  \; & \;                58.2(2)                  \; & \;                44.9(2)                  \; & \;                 12.(2)                  \; & \;               -24.4(4)                  \\ 
 %--------------------------------------------------
 \hline 
              \de_{\QCD,\veto}^{\mu = \MZ}/\% \; & \;                34.7(2)                  \; & \;                40.5(2)                  \; & \;                33.4(2)                  \; & \;                10.0(3)                  \; & \;               -49.1(4)                  \; & \;               -99.6(4)                  \\ 
           \de_{\QCD,\veto}^{\mathrm{var}}/\% \; & \;                26.9(2)                  \; & \;                33.2(4)                  \; & \;                32.7(1)                  \; & \;                23.4(3)                  \; & \;                -7.5(3)                  \; & \;               -45.1(4)                  \\ 
 %--------------------------------------------------
 %--------------------------------------------------
  \hline \hline 
               \de_{\ga,\born}^{\mu = \MZ}/\% \; & \;              0.2264(7)                  \; & \;              0.3036(9)                  \; & \;               0.368(1)                  \; & \;               0.441(1)                  \; & \;               0.564(3)                  \; & \;               0.667(3)                  \\ 
            \de_{\ga,\born}^{\mathrm{var}}/\% \; & \;              0.2562(7)                  \; & \;               0.385(1)                  \; & \;               0.538(1)                  \; & \;               0.743(3)                  \; & \;               1.093(5)                  \; & \;                1.32(1)                  \\ 
 %--------------------------------------------------
 \hline 
                \de_{\ga,\NLO}^{\mu = \MZ}/\% \; & \;              0.2264(7)                  \; & \;              0.3036(9)                  \; & \;               0.368(1)                  \; & \;               0.441(1)                  \; & \;               0.564(3)                  \; & \;               0.667(3)                  \\ 
             \de_{\ga,\NLO}^{\mathrm{var}}/\% \; & \;              0.2562(7)                  \; & \;               0.385(1)                  \; & \;               0.538(1)                  \; & \;               0.743(3)                  \; & \;               1.093(5)                  \; & \;                1.32(1)                  \\ 
 %--------------------------------------------------
 \hline \hline
 %          \de_{\ga,\NLO,\veto}^{\mu = \MZ}/\% \; & \;              0.2264(7)                  \; & \;              0.3036(9)                  \; & \;               0.368(1)                  \; & \;               0.441(1)                  \; & \;               0.564(3)                  \; & \;               0.667(3)                  \\ 
 %       \de_{\ga,\NLO,\veto}^{\mathrm{var}}/\% \; & \;              0.2562(7)                  \; & \;               0.385(1)                  \; & \;               0.538(1)                  \; & \;               0.743(3)                  \; & \;               1.093(5)                  \; & \;                1.32(1)                  \\ 
 % %--------------------------------------------------
 % %--------------------------------------------------
 %  \hline \hline 
 %                    \de_{\Int}^{\mu = \MZ}/\% \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \\ 
 %                 \de_{\Int}^{\mathrm{var}}/\% \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \\ 
 % %--------------------------------------------------
 % \hline 
 %              \de_{\Int,\veto}^{\mu = \MZ}/\% \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \\ 
 %           \de_{\Int,\veto}^{\mathrm{var}}/\% \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \\ 
 % %--------------------------------------------------
 % %--------------------------------------------------
     \si_{\full,\veto}^{\mathrm{var}}/\pba/\% \; & \;                53.1(1)                  \; & \;                7.93(2)                  \; & \;               0.937(1)                  \; & \;              0.0788(3)                  \; & \;             0.00134(2)                  \; & \;           0.0000169(9)                  \\ 
\end{array}$$

==> TotCS-ptl-cuts_ZNul_LHC33_mstw.dat.tex <==
 % Total cs for different cuts at the LHC       
 %************************************************
 % PDFs : mstw
 % p_{\rT,miss}^{\mathrm{min}}/(\GeV)            &                 50.0 &                100.0 &                200.0 &                400.0 &               1000.0 &               2000.0 \\ 
 %-------------------------------------------------
                                                                                                                                      $$ \begin{array}{c|rrrrrr}
                                                                  \multicolumn{7}{c}{\Pp\Pp
                                                                    \to l^+l^-\; \mathrm{jet} + X \;\mbox{at} \;\sqrt{s} =33 \TeV} \\
              \hline p_{\rT,l^+} / \GeV & 50-\infty \;\;\; & 100-\infty \;\;\; & 200-\infty \;\; & 400-\infty \;\; & 1000-\infty \;\; & 2000-\infty \; \\ 
 \hline \hline 
                 \si_{\born}^{\mu = \MZ}/\pba \; & \;              138.38(2)                  \; & \;              12.641(2)                  \; & \;              1.7316(3)                  \; & \;             0.19986(3)                  \; & \;            0.006439(1)                  \; & \;          0.00023702(5)                  \\ 
              \si_{\born}^{\mathrm{var}}/\pba \; & \;              138.01(2)                  \; & \;              12.011(2)                  \; & \;              1.4856(2)                  \; & \;             0.14747(2)                  \; & \;           0.0037329(7)                  \; & \;          0.00011702(2)                  \\ 
 %--------------------------------------------------
 %--------------------------------------------------
  \hline \hline 
                   \de_{\EW}^{\mu = \MZ} / \% \; & \;               -6.99(1)                  \; & \;               -9.26(2)                  \; & \;              -13.57(7)                  \; & \;              -19.96(7)                  \; & \;               -31.0(2)                  \; & \;               -37.1(3)                  \\ 
    \de_{\EW}^{\mathrm{rec}\,,\mu = \MZ} / \% \; & \;               -3.97(9)                  \; & \;               -6.11(4)                  \; & \;              -10.14(5)                  \; & \;              -16.12(9)                  \; & \;               -25.8(2)                  \; & \;               -31.7(2)                  \\ 
 %--------------------------------------------------
 \hline 
                  \de_{\EW}^{\mathrm{var}}/\% \; & \;               -7.00(1)                  \; & \;               -9.08(2)                  \; & \;              -13.18(3)                  \; & \;              -19.11(6)                  \; & \;               -26.7(3)                  \; & \;                -31.(2)                  \\ 
   \de_{\EW}^{\mathrm{rec}\,,\mathrm{var}}/\% \; & \;               -4.12(8)                  \; & \;               -5.82(5)                  \; & \;               -9.65(4)                  \; & \;              -15.07(7)                  \; & \;               -21.8(3)                  \; & \;               -23.3(7)                  \\ 
 %--------------------------------------------------
 %--------------------------------------------------
  \hline \hline 
                    \de_{\QCD}^{\mu = \MZ}/\% \; & \;                32.3(2)                  \; & \;                56.3(2)                  \; & \;                49.6(2)                  \; & \;                28.4(3)                  \; & \;               -21.4(2)                  \; & \;               -67.9(3)                  \\ 
                 \de_{\QCD}^{\mathrm{var}}/\% \; & \;                30.5(2)                  \; & \;                53.2(2)                  \; & \;                51.7(2)                  \; & \;                42.0(2)                  \; & \;                15.9(2)                  \; & \;               -15.1(7)                  \\ 
 %--------------------------------------------------
 \hline 
              \de_{\QCD,\veto}^{\mu = \MZ}/\% \; & \;                 7.9(2)                  \; & \;                22.5(3)                  \; & \;                17.3(1)                  \; & \;                -1.9(2)                  \; & \;               -46.4(2)                  \; & \;               -89.9(3)                  \\ 
           \de_{\QCD,\veto}^{\mathrm{var}}/\% \; & \;                 7.7(2)                  \; & \;                23.4(2)                  \; & \;                25.5(3)                  \; & \;                19.8(1)                  \; & \;                 -1.(1)\times 10^  1     \; & \;               -35.4(6)                  \\ 
 %--------------------------------------------------
 %--------------------------------------------------
  \hline \hline 
               \de_{\ga,\born}^{\mu = \MZ}/\% \; & \;              0.1204(3)                  \; & \;              0.3068(8)                  \; & \;               0.426(1)                  \; & \;               0.525(1)                  \; & \;               0.683(3)                  \; & \;               0.817(3)                  \\ 
            \de_{\ga,\born}^{\mathrm{var}}/\% \; & \;              0.1284(4)                  \; & \;               0.355(1)                  \; & \;               0.559(1)                  \; & \;               0.792(2)                  \; & \;               1.200(4)                  \; & \;               1.498(7)                  \\ 
 %--------------------------------------------------
 \hline \hline
 %                \de_{\ga,\NLO}^{\mu = \MZ}/\% \; & \;              0.1204(3)                  \; & \;              0.3068(8)                  \; & \;               0.426(1)                  \; & \;               0.525(1)                  \; & \;               0.683(3)                  \; & \;               0.817(3)                  \\ 
 %             \de_{\ga,\NLO}^{\mathrm{var}}/\% \; & \;              0.1284(4)                  \; & \;               0.355(1)                  \; & \;               0.559(1)                  \; & \;               0.792(2)                  \; & \;               1.200(4)                  \; & \;               1.498(7)                  \\ 
 % %--------------------------------------------------
 % \hline 
 %          \de_{\ga,\NLO,\veto}^{\mu = \MZ}/\% \; & \;              0.1204(3)                  \; & \;              0.3068(8)                  \; & \;               0.426(1)                  \; & \;               0.525(1)                  \; & \;               0.683(3)                  \; & \;               0.817(3)                  \\ 
 %       \de_{\ga,\NLO,\veto}^{\mathrm{var}}/\% \; & \;              0.1284(4)                  \; & \;               0.355(1)                  \; & \;               0.559(1)                  \; & \;               0.792(2)                  \; & \;               1.200(4)                  \; & \;               1.498(7)                  \\ 
 % %--------------------------------------------------
 % %--------------------------------------------------
 %  \hline \hline 
 %                    \de_{\Int}^{\mu = \MZ}/\% \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \\ 
 %                 \de_{\Int}^{\mathrm{var}}/\% \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \\ 
 % %--------------------------------------------------
 % \hline 
 %              \de_{\Int,\veto}^{\mu = \MZ}/\% \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \\ 
 %           \de_{\Int,\veto}^{\mathrm{var}}/\% \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;    
%           0.0000(0)                  \; & \;              0.0000(0)                  \\ 
 %--------------------------------------------------
 %--------------------------------------------------
     \si_{\full,\veto}^{\mathrm{var}}/\pba/\% \; & \;               139.2(3)                  \; & \;               13.78(2)                  \; & \;               1.677(4)                  \; & \;              0.1497(3)                  \; & \;              0.0025(7)                  \; & \;            0.000041(2)                  \\ 
\end{array}$$
